Differentiating a Tensor Language

How does one compile derivatives of tensor programs, such that the resulting code is purely functional (hence easier to optimize and parallelize) and provably efficient relative to the original program? We show that naively differentiating tensor code---as done in popular systems like Tensorflow and PyTorch---can cause asymptotic slowdowns in pathological cases, violating the Cheap Gradients Principle. However, all existing automatic differentiation methods that guarantee this principle (for variable size data) do so by relying on += mutation through aliases/pointers---which complicates downstream optimization. We provide the first purely functional, provably efficient, adjoint/reverse-mode derivatives of array/tensor code by explicitly accounting for sparsity. We do this by focusing on the indicator function from Iverson's APL. We also introduce a new "Tensor SSA" normal form and a new derivation of reverse-mode automatic differentiation based on the universal property of inner-products.

==> fig/adjoint_id.tex <==

\begin{figure}[t]
\begingroup
\newcommand{\I}{\inner}
\newcommand{\+}{\mplus}
\newcommand{\0}{\mzero}
\newcommand{\E}[1]{%
  \color{meta}\left\llbracket
    \normalcolor #1
  \color{meta}\right\rrbracket
    \normalcolor
}
\arraycolsep=1.8pt
%\centering
\begin{framed}
Grammar Extension
\begin{align*}
L  ::= &~\mwd{let} dx \meq e \mwd{in} L ~|~ \kwd{let} x \keq e \kwd{in} L ~|~ S \\
S  ::= &~\ I \+ S ~|~ I \\
I  ::= &~\msum_{i=0}^n I ~~|~ \I{e}{e} ~|~ \I{e}{e}_{\!\msub{p}} ~|~ \0 
\end{align*}
%
Semantics via de-sugaring
\begin{align*}
%
%
\E{\mwd{let} dx \meq e \mwd{in} L}  &\to \kwd{let} dx \keq e \kwd{in} \E{L} \\
\E{I \+ S}                          &\to \E{I} + \E{S} \\
\E{\msum_{i=0}^n I}                 &\to \ssum_{i=0}^n \E{I} \\
\E{\I{e_0}{e_1}}                    &\to e_0 \cdot e_1                  &(e_0,e_1 : \R) \\
\E{\I{e_0}{e_1}}                    &\to \E{\I{\pi_0~e_0}{\pi_0~e_1}} +
                                         \E{\I{\pi_1~e_0}{\pi_1~e_1}}   &(e_0,e_1:(T_0,T_1)) \\
\E{\I{e_0}{e_1}_{\!\msub{p}}}       &\to \ssum_{\harpoon\imath}^n \ind{p}\cdot
                                            \E{\I{e_0[\harpoon\imath]}{e_1[\harpoon\imath]}}
                                                                        &(e_0,e_1:[n_0,\hdots,n_k]T) \\
\end{align*}
\end{framed}
\caption{Adjoint Approach for Tensors via inner products; Without derivatives, detecting the linear components (e.g. see rule for products) is complicated.}
\label{fig:adjoint_id}
\endgroup
\end{figure}


==> tex/08_design_discussion.tex <==


\subsection{Limitations and Possible Alternatives}

The formal cost model we use is not reflective of the cost of accessing memory, which is substantial in real systems.

This is true.  However, consider the alternative of costing reads and/or writes.  This cost would not be preserved in the transformation to tensor SSA because a code-size-proportional number of intermediate buffers are introduced.  (1) What we have revealed is that such a cost model dis-counts the intermediate values in non-SSA code by presuming that they are stored in ``registers'' or something similar.  (2) Generalizing this insight, the actual cost of reads/writes is not well-reflected by a simple count, but rather depends on \emph{locality} in the way data is accessed.  (3) Now observe that irrespective of the conversion to Tensor SSA, adjoint differentiation necessarily introduces many long-range dependencies, which is why Griewank observes (even in the case of scalar code) that there is no analogous cost bound on memory consumption.  Therefore, while a better theoretical cost model could account for reads and writes, it would inevitably conflict with the spirit of Griewank's original argument.  This more empirically accurate yardstick would therefore (and counter-intuitively) deny us the ability to analyze a non-trivial claim that our auto-diff system preserves work and parallelism complexity measures.


